Learning to Cache With No Regrets

This paper introduces a novel caching analysis that, contrary to prior work, makes no modeling assumptions for the file request sequence. We cast the caching problem in the framework of Online Linear Optimization (OLO), and introduce a class of minimum regret caching policies, which minimize the losses with respect to the best static configuration in hindsight when the request model is unknown. These policies are very important since they are robust to popularity deviations in the sense that they learn to adjust their caching decisions when the popularity model changes. We first prove a novel lower bound for the regret of any caching policy, improving existing OLO bounds for our setting. Then we show that the Online Gradient Ascent (OGA) policy guarantees a regret that matches the lower bound, hence it is universally optimal. Finally, we shift our attention to a network of caches arranged to form a bipartite graph, and show that the Bipartite Subgradient Algorithm (BSA) has no regret

==> related_works_V5.tex <==
 
Other notable  approaches learn the  instantaneous popularity model with no prior assumptions. For instance \cite{gunduz-reinforcement,giannakis-q-learning} employ 
\emph{Q-learning}, and \cite{mihaela-video-caching} leverages a scalable prediction approach; but contrary to this paper, they all assume that the evolution of popularity is  stationary across time. The design of adaptive paging policies is systematically studied  in \cite{geulen2010regret,englert2013economical, lykouris-ML} as an online learning problem. These works differ from our approach since they consider the paging problem, i.e., hit ratio maximization when caching entire files in a single cache. 


Caching networks (CNs) on the other hand, are hitherto under-explored, yet very important as in most cases caches are organized in networks. In CNs one needs to jointly decide which cache will satisfy a request (routing) and which files will be evicted (caching). The work \cite{ioannidis_icn17} introduced a joint routing and caching  algorithm for general graphs, assuming however that file popularity is stationary. On the other hand, \cite{giovanidis-mLRU} proposed the multi-LRU (mLRU) heuristic strategy, and \cite{leonardi-implicit} proposed the ``lazy rule'' extending $q$-LRU to provide local optimality guarantees under stationary requests. \emph{It transpires that we currently lack a principled method to design caching policies with provable performance guarantees, under general popularity conditions, for single or networks of caches. This is exactly the focus of our work.}

%Beyond stationary requests, the problem of online joint routing and caching remains open. 
